Natural Gradient Interpretation of Rank-One Update in CMA-ES

The covariance matrix adaptation evolution strategy (CMA-ES) is a stochastic search algorithm using a multivariate normal distribution for continuous black-box optimization. In addition to strong empirical results, part of the CMA-ES can be described by a stochastic natural gradient method and can be derived from information geometric optimization (IGO) framework. However, there are some components of the CMA-ES, such as the rank-one update, for which the theoretical understanding is limited. While the rank-one update makes the covariance matrix to increase the likelihood of generating a solution in the direction of the evolution path, this idea has been difficult to formulate and interpret as a natural gradient method unlike the rank-$\mu$ update. In this work, we provide a new interpretation of the rank-one update in the CMA-ES from the perspective of the natural gradient with prior distribution. First, we propose maximum a posteriori IGO (MAP-IGO), which is the IGO framework extended to incorporate a prior distribution. Then, we derive the rank-one update from the MAP-IGO by setting the prior distribution based on the idea that the promising mean vector should exist in the direction of the evolution path. Moreover, the newly derived rank-one update is extensible, where an additional term appears in the update for the mean vector. We empirically investigate the properties of the additional term using various benchmark functions.

==> 02_body/04_mapcma.tex <==
\color{blue}
% ========================================
\section{Maximum a Posteriori CMA-ES} \label{sec:mapcma}
% ========================================
In this section, we propose maximum a posteriori CMA-ES~(MAP-CMA). The MAP-CMA employs the rank-$\mu$ update incorporating the prior information derived from the MAP-IGO. In this study, the normal-inverse-Wishart distribution, the conjugate prior of the multivariate normal distribution, is applied to the prior of the MAP-IGO. The natural gradient of the log-likelihood of the normal-inverse-Wishart distribution is then computed to derive the extended rank-$\mu$ update.

\subsection{Natural Gradient for Normal-Inverse-Wishart Distribution}
The normal-inverse-Wishart distribution is defined by
\begin{align}
    p(\btheta) = \mathcal{N} \left( \boldsymbol{m} \mid \boldsymbol{\delta}, \frac{1}{\gamma} \boldsymbol{C} \right) \mathcal{W}^{-1} ( \boldsymbol{C} \mid \PSI, \nu) \enspace.
\end{align}
In the normal-inverse-Wishart distribution, the multivariate normal distribution is given as
\begin{align*}
    \mathcal{N} \left( \boldsymbol{m} \mid \boldsymbol{\delta}, \frac{1}{\gamma} \boldsymbol{C} \right) =  \left( \frac{\gamma}{2\pi} \right)^{\frac{N}{2}} |\boldsymbol{C}|^{-\frac12} \exp \left( -\frac{\gamma}{2} (\boldsymbol{m} - \boldsymbol{\delta})^\top \boldsymbol{C}^{-1} (\boldsymbol{m} - \boldsymbol{\delta}) \right) \:,
\end{align*}
where $\boldsymbol{\delta} \in \R^N$ and $\gamma > 0$. The inverse-Wishart distribution is given as
\begin{align*}
    \mathcal{W}^{-1} ( \boldsymbol{C} \mid \PSI, \nu) = \frac{|\PSI|^{\frac{\nu}{2}}}{2^{\frac{\nu N}{2}}\Gamma_N \left( \frac{\nu}{2} \right)} |\boldsymbol{C}|^{-\frac{\nu + N + 1}{2}}  \exp\left( - \frac12 \Tr \left( \PSI \boldsymbol{C}^{-1} \right) \right) \enspace,
\end{align*}
where $\Gamma_N (\cdot)$ is the multivariate gamma function, $\nu > N-1$, and $\PSI \in \R^{N \times N}$ is a positive define matrix.

We derive the natural gradient of the log-likelihood of the normal-inverse-Wishart distribution over the parameter space of the multivariate normal distribution.
% Let $\btheta = [\boldsymbol{m}^\top, \VEC (\boldsymbol{C})^\top ]^\top$, where $\VEC (\boldsymbol{C})$ represents the matrix $\boldsymbol{C}$ rearranged into a column vector. This parameterization can be found in \cite{Akimoto:2010}.
Let $\btheta = [\boldsymbol{m}^\top, \VEC (\boldsymbol{C})^\top ]^\top$.
The vanilla gradient of the log-likelihood of $p(\btheta)$ is given as follows:
\begin{align}
    \nabla_\btheta \ln p(\btheta) = \left[
    \begin{array}{c}
        -\gamma \boldsymbol{C}^{-1} (\boldsymbol{m} - \boldsymbol{\delta}) \\[5pt]
        \begin{aligned}
            &\frac12 \VEC \left( \gamma \boldsymbol{C}^{-1} (\boldsymbol{m} - \boldsymbol{\delta}) (\boldsymbol{m} - \boldsymbol{\delta})^\top  \boldsymbol{C}^{-1} \right. \\
            &\qquad\quad \left. - (\nu + N + 2) \boldsymbol{C}^{-1} + \boldsymbol{C}^{-1} \PSI \boldsymbol{C}^{-1} \right)
        \end{aligned}
    \end{array}
    \right] \enspace.
\end{align}
According to \cite{Akimoto:2010}, the Fisher information matrix $F(\btheta)$ of the multivariate normal distribution and its inverse matrix are, respectively,
\begin{align*}
    F(\btheta) = \left[
    \begin{array}{cc}
        \boldsymbol{C}^{-1} & \boldsymbol{0} \\
        \boldsymbol{0} & \frac12 \boldsymbol{C}^{-1} \otimes \boldsymbol{C}^{-1}
    \end{array}
    \right] \enspace \text{and} \enspace F^{-1}(\btheta) = \left[
    \begin{array}{cc}
        \boldsymbol{C} & \boldsymbol{0} \\
        \boldsymbol{0} & 2 \boldsymbol{C} \otimes \boldsymbol{C}
    \end{array}
    \right] ,
\end{align*}
where $\otimes$ is the Kronecker product. Hence, the natural gradient of the log-likelihood of $p(\btheta)$ is calculated as follows:
\begin{align}
    \ngr_\btheta \ln p(\btheta) = \left[
    \begin{array}{c}
        -\gamma (\boldsymbol{m} - \boldsymbol{\delta}) \\
        \VEC \left( \gamma (\boldsymbol{m} - \boldsymbol{\delta}) (\boldsymbol{m} - \boldsymbol{\delta})^\top + \PSI - (\nu + N + 2) \boldsymbol{C} \right)
    \end{array}
    \right] \enspace.
\end{align}

\subsection{Update Rules for MAP-CMA}
From \cite{Akimoto:2010}, the natural gradient of the log-likelihood of $p_\btheta (x)$ is calculated as
\begin{align}
    \ngr_\btheta \ln p_\btheta (\x) = \left[
    \begin{array}{c}
        (\x - \boldsymbol{m}) \\
        \VEC \left( (\x - \boldsymbol{m})(\x - \boldsymbol{m})^\top - \boldsymbol{C} \right)
    \end{array}
    \right] \enspace.
\end{align}
Let $\w_i = \hat{\w}_i / (\sum_{j=1}^\lambda \hat{\w}_j )$ for short, and we obtain the extended rank-$\mu$ update rule from Eq.~\eqref{eq:MAP-IGO-update}.
\begin{align*}
    \m[t+1] &= \m[t] + c_m \left( \sum_{i=1}^\lambda \w_i (\x_{i:\lambda} - \m[t] ) - \gamma (\m[t] - \boldsymbol{\delta})  \right) \enspace, \\
    \C[t+1] &= \C[t] + c_\mu \Biggl( \sum_{i=1}^\lambda \w_i \left( (\x_{i:\lambda} - \m[t])(x_{i:\lambda} - \m[t])^\top - \C[t] \right) \Biggr. \notag \\
    &\qquad\qquad\qquad\quad \Biggl. + \gamma (\m[t] - \boldsymbol{\delta}) (\m[t] - \boldsymbol{\delta})^\top + \Psi - (\nu + N + 2) \C[t] \Biggr) \enspace.
\end{align*}
Then, the MAP-CMA is obtained by combining this extended rank-$\mu$ update, the rank-one update, and the step-size adaptation. The single update in the MAP-CMA-ES is shown in Algorithm~\ref{alg:proposed}. \colorbox[gray]{0.90}{Shaded areas} are differences from the original CMA-ES and represent terms corresponding to the natural gradient of the log-likelihood of the prior distribution. When the parameters of the prior distribution are set so that these natural gradient terms are zero vector or zero matrix, i.e., $\boldsymbol{\delta} = \m[t]$, $\PSI = (\nu + N + 2)\C[t]$, the MAP-CMA coincides with the original CMA-ES.

\begin{comment}
{
\setlength{\algomargin}{0.1em}
\begin{algorithm}[t]
    \caption{Single update in MAP-CMA-ES}
    \label{alg:proposed}
    \begin{algorithmic}[1]
        \STATE \textbf{given } $\m[t] \in \R^N$, $\sig[t] \in \R_{+}$, $\C[t] \in \R^{N \times N}$, $\ps[t] \in \R^N$, $\pc[t] \in \R^N$, $\gamma \in \R$, $\boldsymbol{\delta} \in \R^N$, $\PSI \in \R^{N \times N}$, $\nu \in \R$
        \FOR {$i = 1, \ldots, \lambda$}
            \STATE $\y_i \sim \mathcal{N}(\boldsymbol{0}, \C[t])$
            \STATE $\x_i \leftarrow \m[t] + \sig[t] \y_i$
        \ENDFOR
        \STATE Sort $\{\x_{1:\lambda}, \x_{2:\lambda}, \ldots, \x_{\lambda:\lambda}\}$ and $\{\y_{1:\lambda}, \y_{2:\lambda}, \ldots, \y_{\lambda:\lambda}\}$ so that the indices correspond to $f(\x_{1:\lambda}) \leq f(\x_{2:\lambda}) \leq \ldots \leq f(\x_{\lambda:\lambda})$
        \STATE $\m[t+1] \leftarrow \m[t] + c_{m} \left( \sum_{i=1}^{\lambda} w_{i} ( \x_{i:\lambda} - \m[t] ) \highlight{- \gamma (\m[t] - \boldsymbol{\delta}) \hspace{-2pt} } \right)$
        \STATE $\ps[t+1] \leftarrow (1-c_\sigma)\ps[t] + \sqrt{c_\sigma(2-c_\sigma)\muw} {\C[t]}^{-\frac12} \sum_{i=1}^\lambda \w_i \y_{i:\lambda}$
        \STATE $h_\sigma \leftarrow \mathds{1} {\{\|\ps[t+1]\| < \sqrt{1-(1-c_\sigma)^{2(t+1)}}\left(1.4+\frac{2}{N+1}\right)\E [\|\mathcal{N}(\boldsymbol{0}, \mathbf{I}) \|]\}}$
        %\STATE $h_\sigma \leftarrow \begin{cases} 1 \enspace \text{if} \enspace \|\ps[t+1]\|^2 < \sqrt{1-(1-c_\sigma)^{2(t+1)}}\left(1.4+\frac{2}{N+1}\right)\E [\|\mathcal{N}(\boldsymbol{0}, \mathbf{I}) \|] \\ 0 \end{cases}$
        \STATE $\pc[t+1] \leftarrow (1-c_c) \pc[t] + h_\sigma \sqrt{c_c(2-c_c)\muw} \sum_{i=1}^\lambda \w_i \y_{i:\lambda}$
        % {\thickmuskip=0mu
        % \medmuskip=0mu
        % \thinmuskip=0mu
        % \STATE $\C[t+1] \leftarrow \left(1 + (1-h_\sigma)c_1 c_c(2-c_c) \right) \C[t] $\linebreak $+ \underbrace{c_1 \left( \pc[t+1]{\pc[t+1]}^\top - \C[t] \right) }_{\text{rank-one update}}$\linebreak $ + \underbrace{c_\mu \left( \sum_{i=1}^\lambda w_i \left(\y_{i:\lambda}\y_{i:\lambda}^\top - \C[t]\right) \highlight{ +\gamma (\m[t] - \boldsymbol{\delta}) (\m[t] - \boldsymbol{\delta})^\top + \PSI - (\nu + N + 2)\C[t] \hspace{-3pt} } \hspace{-1pt} \right)}_{\text{rank-}\mu\text{ update}}$
        % }
        {
        \STATE $\C[t+1] \leftarrow \left(1 + (1-h_\sigma)c_1 c_c(2-c_c) \right) \C[t] $\linebreak $\ +\ c_1 \left( \pc[t+1]{\pc[t+1]}^\top - \C[t] \right)
        \ +\ c_\mu \Bigl( \sum_{i=1}^\lambda w_i \left(\y_{i:\lambda}\y_{i:\lambda}^\top - \C[t]\right)$\linebreak
        \null\quad\quad $\highlight{ +\gamma (\m[t] - \boldsymbol{\delta}) (\m[t] - \boldsymbol{\delta})^\top + \PSI - (\nu + N + 2)\C[t] \hspace{-1pt} } \Bigr)$
        }        
        \STATE $\sig[t+1] \leftarrow \sig[t] \exp \left( \frac{c_\sigma}{d_\sigma} \left( \frac{\|\ps[t+1] \|}{\E [\|\mathcal{N}(\boldsymbol{0}, \mathbf{I}) \|]} - 1 \right) \right)$
    \end{algorithmic}
\end{algorithm}
}
\end{comment}

\begin{algorithm}[t]
    \caption{Single update in the MAP-CMA}
    \label{alg:proposed}
    \begin{algorithmic}[1]
        \STATE \textbf{given } $\m[t] \in \R^N$, $\sig[t] \in \R_{+}$, $\C[t] \in \R^{N \times N}$, $\ps[t] \in \R^N$, $\pc[t] \in \R^N$, $\gamma \in \R$, $\boldsymbol{\delta} \in \R^N$, $\PSI \in \R^{N \times N}$, $\nu \in \R$
        \FOR {$i = 1, \ldots, \lambda$}
            \STATE $\y_i \sim \mathcal{N}(\boldsymbol{0}, \C[t])$
            \STATE $\x_i \leftarrow \m[t] + \sig[t] \y_i$
        \ENDFOR
        % \STATE Sort $\{\x_{1:\lambda}, \x_{2:\lambda}, \ldots, \x_{\lambda:\lambda}\}$ and $\{\y_{1:\lambda}, \y_{2:\lambda}, \ldots, \y_{\lambda:\lambda}\}$ so that the indices correspond to $f(\x_{1:\lambda}) \leq f(\x_{2:\lambda}) \leq \ldots \leq f(\x_{\lambda:\lambda})$
        \STATE $\ps[t+1] \leftarrow (1-c_\sigma)\ps[t] + \sqrt{c_\sigma(2-c_\sigma)\muw} {\C[t]}^{-\frac12} \sum_{i=1}^\lambda \w_i \y_{i:\lambda}$
        % \STATE $h_\sigma \leftarrow \mathds{1} {\{\|\ps[t+1]\| < \sqrt{1-(1-c_\sigma)^{2(t+1)}}\left(1.4+\frac{2}{N+1}\right)\E [\|\mathcal{N}(\boldsymbol{0}, \mathbf{I}) \|]\}}$
        \STATE $\pc[t+1] \leftarrow (1-c_c) \pc[t] + \sqrt{c_c(2-c_c)\muw} \sum_{i=1}^\lambda \w_i \y_{i:\lambda}$
        \STATE $\m[t+1] \leftarrow \m[t] + c_{m} \left( \sum_{i=1}^{\lambda} w_{i} ( \x_{i:\lambda} - \m[t] ) \highlight{- \gamma (\m[t] - \boldsymbol{\delta}) \hspace{-2pt} } \right)$
        \STATE $\C[t+1] \leftarrow \C[t] + c_\mu \Biggl( \sum_{i=1}^\lambda w_i \left(\y_{i:\lambda}\y_{i:\lambda}^\top - \C[t]\right)$\linebreak
        \null\qquad\qquad $\highlight{ + \frac{\gamma}{(\sig[t])^2} (\m[t] - \boldsymbol{\delta}) (\m[t] - \boldsymbol{\delta})^\top + \frac{\Psi}{(\sig[t])^2} - (\nu + N + 2)\C[t] \hspace{-1pt} } \Biggr)$
        \STATE $\sig[t+1] \leftarrow \sig[t] \exp \left( \frac{c_\sigma}{d_\sigma} \left( \frac{\|\ps[t+1] \|}{\E [\|\mathcal{N}(\boldsymbol{0}, \mathbf{I}) \|]} - 1 \right) \right)$
    \end{algorithmic}
\end{algorithm}
\color{black}
